FOND Planning for LTLf and PLTLf Goals

In this report, we will define a new approach to the problem of non deterministic planning for extended temporal goals. In particular, we will give a solution to this problem reducing it to a fully observable non deterministic (FOND) planning problem and taking advantage of the LTLfToDFA tool. First of all, we will introduce the main idea and motivations supporting our approach. Then, we will give some preliminaries explaining the Planning Domain Definition Language (PDDL) language and the FOND planning problem formally. After that, we will illustrate our FOND4LTLfPLTLf (also available online) approach with the encoding of temporal goals into a PDDL domain and problem. Finally, we will present some of the results obtained through the application of the proposed solution.

==> sections/implementation.tex <==
\section{Implementation}\label{sec:planning-implementation}
In this section, we thoroughly describe the proposed implementation of concepts given in Section \ref{sec:fond-plan-appr}. In particular, we give some general information about its features, dependencies and usage. Then, we focus on the package explaining how is structured and commenting highlights on the code. 

We decided to call the package \FONDFOR, enhancing the possibility to solve \FOND planning also for \PLTLf goals, which is a novelty in this area of research and application. Moreover, the package has been developed in pure Python and has the following main features:
\begin{itemize}
\item perform \FOND planning for \LTLf or \PLTLf goals;
\item compiling simple ADL conditional effects from the planning domain;
\item encode \LTLf/\PLTLf formulas into standard \PDDL \citep{mcdermott1998pddl}.
\end{itemize}
These features are achieved together with the integration of the \LTLfToDFA tool (Chapter \ref{ch:ltlf2dfa}).

Secondly, \FONDFOR requires Python>=3.6 and has the following dependencies:
\begin{itemize}
\item \LTLfToDFA, presented in Chapter \ref{ch:ltlf2dfa}. It has been used for the generation of \DFAs corresponding to \LTLf/\PLTLf goal formulas;
\item \href{http://www.dabeaz.com/ply/ply.html}{PLY}, a pure-Python implementation of the popular compiler construction tools \href{http://dinosaur.compilertools.net/}{Lex and Yacc}. It has been employed for \PDDL parsing;
\item \href{https://pypi.org/project/pydot/}{pydot}, a Python interface to GraphViz format language. It has been employed for \DFAs parsing;
\item possible other dependencies linked to the employed planner. In the case of FOND-SAT, it has MINISAT as dependency.
\end{itemize} 
The \FONDFOR software is an open-source project and available to download on GitHub\footnote{https://github.com/Francesco17/FOND4LTLfPLTL}.

Additionally, \FONDFOR will soon be available as an online tool at the website address \href{http://fond4ltlfpltl.diag.uniroma1.it}{http://fond4ltlfpltl.diag.uniroma1.it}.
\subsection{Package Structure}
The structure of the \FONDFOR package is ordered and divided according to the scope of each single module. It consists of the following:
\begin{itemize}
\item \texttt{pddl/}: it is the directory containing all the necessary code for parsing the \PDDL standard and all data structures designed and implemented to handle \PDDL;
\item  \texttt{automa/}: it consists of the \texttt{automa.py} file, the \texttt{aparser.py} file and the \texttt{symbol.py} file. In this folder, we find all the code for dealing with automata;
\item \texttt{fond4ltlfpltl.py}: it is the main module of the package.
\end{itemize}
\subsection{\PDDL}\label{sec:impl-pddl}
In this section, we illustrate the code that handles the \PDDL standard. More specifically, we talk about the parsing of \PDDL domains and problems showing all implemented data structures.

First of all, thanks to the PLY library we have implemented the \texttt{lexer.py} and the \texttt{parser.py} modules enabling the parsing of a \PDDL document. For a brief overview of the functioning of PLY we refer the reader to Sections \ref{sec:lexer} and \ref{sec:parser}. Indeed, the operation is exactly the same. In the following, we show the listing of the two modules focusing only on the most important parts. Three dots $\dots$ represent omitted code.

\begin{lstlisting}[language=Python, style=Python, escapechar = £,  label={code:fond-lexer}, caption={The \texttt{MyLexer} class.}]
import ply.lex as lex

class MyLexer(object):

    reserved = {
        'define':                   'DEFINE_KEY',
        'domain':                   'DOMAIN_KEY',
        ':domain':                  'DOMAIN_PKEY',
        ':requirements':            'REQUIREMENTS_KEY',
        ':constants':               'CONSTANTS_KEY',
        ':strips':                  'STRIPS_KEY',
        ':adl':                     'ADL_KEY',
        ':non-deterministic':       'ND_KEY',
        ':equality':                'EQUALITY_KEY',
        ':typing':                  'TYPING_KEY',
        ':types':                   'TYPES_KEY',
        ':predicates':              'PREDICATES_KEY',
        ':action':                  'ACTION_KEY',
        ':parameters':              'PARAMETERS_KEY',
        ':precondition':            'PRECONDITION_KEY',
        ':effect':                  'EFFECT_KEY',
        'and':                      'AND_KEY',
        'or':                       'OR_KEY',
        'not':                      'NOT_KEY',
        'imply':                    'IMPLY_KEY',
        'oneof':                    'ONEOF_KEY',
        'forall':                   'FORALL_KEY',
        'exists':                   'EXISTS_KEY',
        'when':                     'WHEN_KEY',
        'problem':                  'PROBLEM_KEY',
        ':objects':                 'OBJECTS_KEY',
        ':init':                    'INIT_KEY',
        ':goal':                    'GOAL_KEY'
    }

    tokens = (
         'NAME',
         'VARIABLE',
         'LPAREN',
         'RPAREN',
         'HYPHEN',
         'EQUALS'
    ) + tuple(reserved.values())

    t_LPAREN = r'\('
    t_RPAREN = r'\)'
    t_HYPHEN = r'\-'
    t_EQUALS = r'='

    t_ignore = ' \t'

    def t_KEYWORD(self, t):
        r':?[a-zA-z_][a-zA-Z_0-9\-]*'
        t.type = self.reserved.get(t.value,'NAME')
        return t

    def t_NAME(self, t):
        r'[0-9a-zA-z_][a-zA-Z_0-9\-]*'
        return t

    def t_VARIABLE(self, t):
        r'\?[a-zA-z_][a-zA-Z_0-9\-]*'
        return t

    def t_COMMENT(self, t):
        r';.*'
        pass
...
    def t_newline(self, t):
        r'\n+'
        t.lineno += len(t.value)
...
\end{lstlisting}
As we can see, we have defined all tokens present in \PDDL plus the \textit{oneof} keyword, which is used to parse also non deterministic actions. Then, we have specified all regular expression rules for those tokens.

On the other hand, following the official \PDDL standard grammar syntax, we have implemented the \texttt{MyParser} class as follows:

\begin{lstlisting}[language=Python, style=Python, escapechar = £,  label={code:fond-parser}, caption={The \texttt{MyParser} class.}]
...
class MyParser(object):
...

    def p_pddl(self, p):
        '''pddl : domain
                 | problem'''
        p[0] = p[1]

    def p_domain(self, p):
        '''domain : LPAREN DEFINE_KEY domain_def require_def types_def 
        constants_def predicates_def action_def_lst RPAREN
                   | LPAREN DEFINE_KEY domain_def require_def types_def 
                   predicates_def action_def_lst RPAREN
                   | LPAREN DEFINE_KEY domain_def require_def predicates_def 
                   action_def_lst RPAREN'''
        if len(p) == 10:
            p[0] = Domain(p[3], p[4], p[5], p[6], p[7], p[8])
        elif len(p) == 9:
            p[0] = Domain(p[3], p[4], p[5], [], p[6], p[7])
        else:
            p[0] = Domain(p[3], p[4], [], [], p[5], p[6])

    def p_problem(self, p):
        '''problem : LPAREN DEFINE_KEY problem_def domain_pdef objects_def 
        init_def goal_def RPAREN'''
        p[0] = Problem(p[3], p[4], p[5], p[6], p[7])
...
    def p_init_def(self, p):
        '''init_def : LPAREN INIT_KEY LPAREN AND_KEY ground_predicates_lst 
        RPAREN RPAREN
                     | LPAREN INIT_KEY ground_predicates_lst RPAREN'''
        if len(p) == 5:
            p[0] = p[3]
        elif len(p) == 8:
            p[0] = p[5]

    def p_goal_def(self, p):
        '''goal_def : LPAREN GOAL_KEY LPAREN AND_KEY ground_predicates_lst 
        RPAREN RPAREN
                     | LPAREN GOAL_KEY ground_predicates_lst RPAREN'''
        if len(p) == 7:
            p[0] = p[5]
        else:
            p[0] = p[3]
...
    def p_predicates_def(self, p):
        '''predicates_def : LPAREN PREDICATES_KEY predicate_def_lst RPAREN
        '''
        p[0] = p[3]
        
    def p_predicate_def(self, p):
        '''predicate_def : LPAREN NAME typed_variables_lst RPAREN
                           | LPAREN NAME RPAREN'''
        if len(p) == 4:
            p[0] = Predicate(p[2])
        elif len(p) == 5:
            p[0] = Predicate(p[2], p[3])
...
    def p_action_def(self, p):
        '''action_def : LPAREN ACTION_KEY NAME parameters_def precond_def 
        effects_def RPAREN'''
        p[0] = Action(p[3], p[4], p[5], p[6])

    def p_parameters_def(self, p):
        '''parameters_def : PARAMETERS_KEY LPAREN typed_variables_lst RPAREN
                            | PARAMETERS_KEY LPAREN RPAREN'''
        if len(p) == 4:
            p[0] = []
        elif len(p) == 5:
            p[0] = p[3]

    def p_precond_def(self, p):
        '''precond_def : PRECONDITION_KEY LPAREN formula RPAREN'''
        p[0] = p[3]

    def p_formula(self, p):
        '''formula : literal
                    | AND_KEY formula_lst
                    | OR_KEY formula_lst
                    | NOT_KEY formula
                    | IMPLY_KEY formula formula
                    | EXISTS_KEY LPAREN typed_variables_lst RPAREN formula
                    | FORALL_KEY LPAREN typed_variables_lst RPAREN formula
                    | LPAREN AND_KEY formula_lst RPAREN
                    | LPAREN OR_KEY formula_lst RPAREN
                    | LPAREN NOT_KEY formula RPAREN
                    | LPAREN IMPLY_KEY formula formula RPAREN
                    | LPAREN literal RPAREN
                    | LPAREN EXISTS_KEY LPAREN typed_variables_lst RPAREN 
                    formula RPAREN
                    | LPAREN FORALL_KEY LPAREN typed_variables_lst RPAREN 
                    formula RPAREN'''
        if len(p) == 2:
            p[0] = p[1]
        elif len(p) == 3:
            if p[1] == 'and':
                p[0] = FormulaAnd(p[2])
            elif p[1] == 'or':
                p[0] = FormulaOr(p[2])
            elif p[1] == 'not':
                p[0] = FormulaNot(p[2])
        elif len(p) == 4:
            if p[1] == 'imply':
                p[0] = FormulaImply(p[2], p[3])
            else:
                p[0] = p[2]
        elif len(p) == 5:
            if p[2] == 'and':
                p[0] = FormulaAnd(p[3])
            elif p[2] == 'or':
                p[0] = FormulaOr(p[3])
            elif p[2] == 'not':
                p[0] = FormulaNot(p[3])
        elif len(p) == 6:
            if p[3] == 'imply':
                p[0] = FormulaImply(p[3], p[4])
            elif p[1] == 'exists':
                p[0] = FormulaExists(p[3], p[5])
            elif p[1] == 'forall':
                p[0] = FormulaForall(p[3], p[5])
        elif len(p) == 8:
            if p[2] == 'exists':
                p[0] = FormulaExists(p[4], p[6])
            elif p[2] == 'forall':
                p[0] = FormulaForall(p[4], p[6])
...
    def p_effects_def(self, p):
        '''effects_def : EFFECT_KEY LPAREN one_eff_formula RPAREN'''
        if p[3] == 'and':
            p[0] = '(and)'
        else:
            p[0] = p[3]

    def p_one_eff_formula(self, p):
        '''one_eff_formula : literal
                             | AND_KEY one_eff_formula_lst
                             | AND_KEY
                             | ONEOF_KEY atomic_eff_lst
                             | WHEN_KEY formula atomic_eff
                             | LPAREN ONEOF_KEY atomic_eff_lst RPAREN
                             | LPAREN WHEN_KEY formula atomic_eff RPAREN
                             | LPAREN FORALL_KEY LPAREN typed_variables_lst 
                             RPAREN atomic_eff RPAREN
                             | LPAREN FORALL_KEY LPAREN typed_variables_lst 
                             RPAREN LPAREN WHEN_KEY formula atomic_eff 
                             RPAREN RPAREN'''
        if len(p) == 2:
            p[0] = p[1]
        elif len(p) == 3:
            if p[1] == 'and':
                p[0] = FormulaAnd(p[2])
            else: p[0] = FormulaOneOf(p[2])
        elif len(p) == 4:
            if p[1] == 'when':
                p[0] = FormulaWhen(p[2], p[3])
        elif len(p) == 5:
            p[0] = FormulaOneOf(p[3])
        elif len(p) == 6:
            p[0] = FormulaWhen(p[3], p[4])
        elif len(p) == 8:
            p[0] = FormulaForall(p[4], p[6])
        elif len(p) == 12:
            nested = FormulaWhen(p[8], p[9])
            p[0] = FormulaForall(p[4], nested)
...
    def p_atomic_eff(self, p):
        '''atomic_eff : literal
                      | AND_KEY literal_lst
                      | LPAREN AND_KEY literal_lst RPAREN
                      | LPAREN WHEN_KEY formula atomic_eff RPAREN'''
        if len(p) == 2:
            p[0] = p[1]
        elif len(p) == 3:
            if p[1] == 'and':
                p[0] = FormulaAnd(p[2])
        elif len(p) == 5:
            if p[2] == 'and':
                p[0] = FormulaAnd(p[3])
        elif len(p) == 6:
            p[0] = FormulaWhen(p[3], p[4])
...
    def p_literal(self, p):
        '''literal : LPAREN NOT_KEY predicate RPAREN
                    | predicate'''
        if len(p) == 2:
            p[0] = Literal.positive(p[1])
        elif len(p) == 5:
            p[0] = Literal.negative(p[3])

    def p_predicate(self, p):
        '''predicate : LPAREN NAME variables_lst RPAREN
                      | LPAREN EQUALS VARIABLE VARIABLE RPAREN
                      | LPAREN NAME RPAREN
                      | NAME variables_lst
                      | EQUALS VARIABLE VARIABLE
                      | NAME'''
        if len(p) == 2:
            p[0] = Predicate(p[1])
        elif len(p) == 3:
            p[0] = Predicate(p[1], p[2])
        elif len(p) == 4:
            if p[1] == '(':
                p[0] = Predicate(p[2])
            else:
                p[0] = Predicate('=', [p[2], p[3]])
        elif len(p) == 5:
            p[0] = Predicate(p[2], p[3])
        elif len(p) == 6:
            p[0] = Predicate('=', [p[3], p[4]])

    def p_typed_variables_lst(self, p):
        '''typed_variables_lst : variables_lst HYPHEN type 
        typed_variables_lst
                                 | variables_lst HYPHEN type'''
        if len(p) == 4:
            p[0] = [Term.variable(name, p[3]) for name in p[1]]
        else:
            p[0] = [Term.variable(name, p[3]) for name in p[1]] + p[4]

    def p_variables_lst(self, p):
        '''variables_lst : VARIABLE variables_lst
                         | VARIABLE'''
        if len(p) == 2:
            p[0] = [p[1]]
        elif len(p) == 3:
            p[0] = [p[1]] + p[2]
...
\end{lstlisting}
In Listing \ref{code:fond-parser}, there are all methods definition that are in charge of constructing the syntax tree structure from tokens found by the lexer in the input string document. Then, we have implemented a data structure for all components belonging to the \PDDL standard, starting from terms and predicates to the whole domain and problem. In this way, we provide a code more manageable and readable.

At this point, we are going to describe one after the other the implemented data structure of the main \PDDL components.

Firstly, variables and constants are represented by the \texttt{Term} class in Listing \ref{code:fond-term}.

\begin{lstlisting}[language=Python, style=Python, escapechar = £,  label={code:fond-term}, caption={The \texttt{Term} class.}]
class Term:

    def __init__(self, **kwargs):
        self._name  = kwargs.get('name',  None)
        self._type  = kwargs.get('type',  None)
        self._value = kwargs.get('value', None)

    @property
    def name(self):
        return self._name

    @property
    def type(self):
        return self._type

    @property
    def value(self):
        return self._value
...
    @classmethod
    def variable(cls, name, type=None):
        return Term(name=name, type=type)

    @classmethod
    def constant(cls, value, type=None):
        return Term(value=value, type=type)

    def __str__(self):
        if self.is_variable() and self.is_typed():
            return '{0} - {1}'.format(self._name, self._type)
        if self.is_variable():
            return '{0}'.format(self._name)
        if self.is_constant() and self.is_typed():
            return '{0} - {1}'.format(self._value, self._type)
        if self.is_constant():
            return '{0}'.format(self._value)
\end{lstlisting}
A \texttt{Term} object is instantiated with three optional arguments: a name, a type and a value, respectively. As said before, a term can represent a variable or a constant. In each of these cases, it handles a possible typing and/or a possible value.

Secondly, we have the \texttt{Predicate} and the \texttt{Literal} classes. The former is used to represent \PDDL fluents, whereas the latter distinguishes between positive and negative fluents. Additionally, the \texttt{Predicate} class can also handle the equality predicates. In the following Listing we propose a glimpse of both the \texttt{Predicate} and the \texttt{Literal} classes.
\begin{lstlisting}[language=Python, style=Python, escapechar = £,  label={code:fond-pred-lit}, caption={The \texttt{Predicate} and the \texttt{Literal} classes.}]
class Predicate:

    def __init__(self, name, args=[]):
        self._name = name
        self._args = args

    @property
    def name(self):
        return self._name

    @property
    def args(self):
        return self._args[:]
...
    def __str__(self):
        if self.name == '=':
            return '(= {0} {1})'.format(str(self._args[0]), 
            str(self._args[1]))
        elif self.arity == 0:
            return '('+self.name+')'
        else:
            return '({0} {1})'.format(self.name, ' '.join(map(str, 
            self._args)))
...

class Literal:

    def __init__(self, predicate, positiveness):
        self.predicate = predicate
        self.positiveness = positiveness
...
    @classmethod
    def positive(cls, predicate):
        return Literal(predicate, True)

    @classmethod
    def negative(cls, predicate):
        return Literal(predicate, False)

    def get_vars(self):
        return self.predicate.args

    def __str__(self):
        if self.is_positive():
            return str(self.predicate)
        if not self.is_positive() and self.predicate.name == '=':
            lhs = str(self.predicate.args[0])
            rhs = str(self.predicate.args[1])
            return '(not (= {0} {1}))'.format(lhs, rhs)
        if not self.is_positive():
            return '(not {})'.format(str(self.predicate))
\end{lstlisting}

After seeing the data structure for low level objects that we have just presented, we are going to illustrate the implementation of data structure for the rest, namely the \texttt{Action} class, the \texttt{Domain} class and, finally, the \texttt{Problem} class. Here, we skip the implementation of each formula since it simply consists of initializing and representing the corresponding object.

Firstly, we show main methods of the \texttt{Action} class in Listing \ref{code:fond-act}.

\begin{lstlisting}[language=Python, style=Python, escapechar = £,  label={code:fond-act}, caption={The \texttt{Action} class.}]
from fond4ltlfpltl.PDDLparser.formula import FormulaAnd, FormulaOneOf
from fond4ltlfpltl.PDDLparser.literal import Literal
from fond4ltlfpltl.PDDLparser.predicate import Predicate

class Action:

    def __init__(self, name, parameters, preconditions, effects):
        self.name = name #string
        self.parameters = parameters #list
        self.preconditions = preconditions #formula.FormulaXXX
        self.effects = effects #formula.FormulaXXX

    def __str__(self):
        operator_str = '{0}\n'.format(self.name)
        operator_str += '\t:parameters ({0})\n'.format(' '.join(map(str, 
        self.parameters)))
        operator_str += '\t:precondition {0}\n'.format(self.preconditions)
        operator_str += '\t:effect {0}\n'.format(self.effects)
        return operator_str

    def add_to_precond(self):
        if isinstance(self.preconditions, FormulaAnd):
            self.preconditions.complete_domain_turn(True)
        else:
            old_formula = self.preconditions
            precond_to_be_added = Literal.positive(Predicate('turnDomain'))
            self.preconditions = FormulaAnd([old_formula,precond_to_be_added])

    def add_to_effect(self):
        if isinstance(self.effects, FormulaAnd):
            self.effects.complete_domain_turn(False)
        else:
            old_formula = self.effects
            effect_to_be_added = Literal.negative(Predicate('turnDomain'))
            self.effects = FormulaAnd([old_formula,effect_to_be_added])

    def add_turn_domain(self):£\label{line:add-turn-domain}£
        self.add_to_precond()
        self.add_to_effect()
\end{lstlisting}

As we can see from the Listing, the \texttt{Action} class contains all main properties, i.e. the name, parameters, preconditions and effects. Moreover, as done for all classes, the \texttt{Action} class has its string representation that convert the operator itself in \PDDL notation. As last remark, notice the \texttt{add\_turn\_domain} method which performs the addition to each operator (except from \texttt{trans} operators) of the domain of the new predicate \texttt{turnDomain}. In particular, we remind the reader that \texttt{turnDomain} is put positive in preconditions and negative on effects.

Secondly, we describe the two main data structures representing \PDDL elements: the \texttt{Domain} class and the \texttt{Problem} class, respectively. Both represent a complete planning task. In Listing \ref{code:fond-dom}, we can see the definition of the \texttt{Domain} class.

\begin{lstlisting}[language=Python, style=Python, escapechar = £,  label={code:fond-dom}, caption={The \texttt{Domain} class.}]
from fond4ltlfpltl.PDDLparser.formula import *
from fond4ltlfpltl.PDDLparser.action import Action
import copy

class Domain:

    def __init__(self, name, requirements, types, constants, predicates, 
    operators):
        self.name = name #string
        self.requirements = requirements #list
        self.types = types #list
        self.constants = constants #list
        self.predicates = predicates #list
        self.operators = operators #list
...
    def add_operators_trans(self, transition_operators):
        for operator in transition_operators:
            self.operators.append(operator)

    def add_predicates(self, parameters, states):
        self.predicates.append('(turnDomain)')
        for state in states:
            self.predicates.append('(q{0} {1})'.format(str(state), 
            ' '.join(map(str, parameters))))
...
    def add_precond_effect(self):
        for op in self.operators:
            op.add_turn_domain()

    def get_new_domain(self, parameters, states, transition_operators):£\label{line:new-dom}£
        self.compile_simple_adl()
        self.add_predicates(parameters, states)
        self.add_precond_effect()
        self.add_operators_trans(transition_operators)
        return self

    def modify_operator(self, op_copy, condition, formula):
        if isinstance(op_copy.preconditions, FormulaAnd):
            op_copy.preconditions.andList.append(condition)
            new_preconditions = op_copy.preconditions.andList
            new_effects = formula
        else:
            new_preconditions = FormulaAnd([op_copy.preconditions,condition])
            new_effects = formula
        new_op = Action(op_copy.name, op_copy.parameters,
         new_preconditions, new_effects)
        return new_op

    def compile_simple_adl(self):£\label{line:compile-adl}£
        i = 0
        for op in self.operators:
            if isinstance(op.effects, FormulaWhen):
                # it remains only one operator, but we need to modify it
                condition_formula = op.effects.condition
                statement_formula = op.effects.formula
                new_op = self.modify_operator(copy.deepcopy(op),
                condition_formula, statement_formula)
                self.operators[i] = new_op
                continue
            elif isinstance(op.effects, FormulaAnd):
                no_of_whens = op.effects.count_whens()
                if no_of_whens == 0:
                    continue
                else:
                    pos = self.operators.index(op)
                    new_op_list = self.split_operator(copy.deepcopy(op),
                    no_of_whens)
                    self.operators[pos:pos+1] = new_op_list
            i +=1

    def split_operator(self, op, number):
        '''
        given a simple adl operator it returns
        a list of operators without adl
        '''
        new_op_list = []
        pair_precond_effect = []
        additionals = []
        formula = op.effects

        for item in formula.andList:
            if isinstance(item, FormulaWhen):
                formula_condition = item.condition
                formula_statement = item.formula
                pair_precond_effect.append([FormulaAnd([op.preconditions,
                formula_condition]), formula_statement])
            else:
                additionals.append(item)
        k = 1
        for j in range(len(pair_precond_effect)):
            pair_precond_effect[j][k] = FormulaAnd([pair_precond_effect[j]
            [k]]+additionals)

        for u in range(number):
            new_op = Action(op.name+'-'+str(u), op.parameters,
             pair_precond_effect[u][0], pair_precond_effect[u][1])
            new_op_list.append(new_op)

        return new_op_list
\end{lstlisting}
As seen in Section \ref{sec:pddl}, a \PDDL domain consists of a name,
the list of requirements, the list of types, the list of constants, the list of predicates and, finally, the list of operators. All items of these list, are instantiations of classes previously seen.
Regarding the \texttt{Domain} class, it comprises a couple of methods that contribute to the creation of the new domain in which we encode temporal goals. Additionally, at line \ref{line:compile-adl}, the class provides a method to compile away simple conditional effects in operators. This functionality simply splits operators containing conditional effects as many times as the number of conditional effects appearing in the action. More specifically, for each conditional effect we put the condition in action's preconditions and leave the effect-formula in the action's effect. Finally, we have the \texttt{get\_new\_domain} method, at line \ref{line:new-dom}, that gathers and invokes all methods for obtaining the new domain with encoded temporal goals.

Finally, we present the \texttt{Problem} class in Listing \ref{code:fond-prob}.

\begin{lstlisting}[language=Python, style=Python, escapechar = £,  label={code:fond-prob}, caption={The \texttt{Problem} class.}]
from fond4ltlfpltl.PDDLparser.formula import FormulaOr

class Problem(object):

    new_goal = set()

    def __init__(self, name, domain, objects, init, goal):
        self._name = name
        self._domain = domain
        self._objects = {}
        for obj in objects:
            self._objects[obj.type] = self._objects.get(obj.type, [])
            self._objects[obj.type].append(str(obj.value))
        self._init = set(map(str, init))
        self._goal = set(map(str, goal))

    @property
    def name(self):
        return self._name

    @property
    def domain(self):
        return self._domain

    @property
    def objects(self):
        return self._objects.copy()

    @property
    def init(self):
        return self._init.copy()

    @property
    def goal(self):
        return self._goal.copy()

    def __str__(self):
        problem_str  = '(define (problem {0})\n'.format(self._name)
        problem_str += '\t(:domain {0})\n'.format(self._domain)
        problem_str += '\t(:objects'
        for type, objects in self._objects.items():
            problem_str += ' {0} - {1}'.format(' '.join(sorted(objects)), 
            type)
        problem_str += ')\n'
        problem_str += '\t(:init {0})\n'.format(' '.join(sorted(
        self._init)))
        problem_str += '(:goal (and {0}))\n'.format(
        ' '.join(sorted(self.new_goal)))
        problem_str += ')'
        return problem_str

    def make_new_init(self, obj_list):£\label{line:new-init}£
        self._init.add('(turnDomain)')
        if obj_list:
            self._init.add('(q1 {0})'.format(' '.join(obj_list)))
        else:
            self._init.add('(q1)')
        return self._init

    def make_new_goal(self, final_states, obj_list):£\label{line:new-goal}£
        self.new_goal.add('(turnDomain)')
        if len(final_states) > 1:
            or_list = []
            for state in final_states:
                if obj_list:
                    or_list.append('(q{0} {1})'.format(str(state), 
                    ' '.join(obj_list)))
                else:
                    or_list.append('(q{0})'.format(str(state)))
            new_formula = FormulaOr(or_list)
            self.new_goal.add(str(new_formula))
        else:
            if obj_list:
                self.new_goal.add('(q{0} {1})'.format(final_states[0], 
                ' '.join(obj_list)))
            else:
                self.new_goal.add('(q{0})'.format(final_states[0]))

    def get_new_problem(self, final_states, symbols_list):£\label{line:new-prob}£
        obj_list = self.extract_object_list(symbols_list)
        self.objects_are_upper(obj_list)
        self.make_new_init(obj_list)
        self.make_new_goal(final_states, obj_list)
        return self

    def extract_object_list(self, symbols_list):
        already_seen = set()
        obj_list = []
        for symbol in symbols_list:
            if symbol.objects:
                for obj in symbol.objects:
                    if obj not in already_seen:
                        already_seen.add(obj)
                        obj_list.append(obj)
                    else:
                        pass
            else:
                continue
        return obj_list

    def objects_are_upper(self, objects):
        for value_list in self.objects.values():
            for val in value_list:
                if val.isupper() and val.lower() in objects:
                    objects[objects.index(val.lower())] = 
                    objects[objects.index(val.lower())].upper()
                else:
                    pass
\end{lstlisting}
The main methods are:
\begin{itemize}
\item \texttt{make\_new\_init} (line \ref{line:new-init});
\item \texttt{make\_new\_goal} (line \ref{line:new-goal});
\item \texttt{get\_new\_problem} (line \ref{line:new-prob}).
\end{itemize}
Having the informations about the \DFA encoding, the first method computes the new initial specification by adding the \texttt{turnDomain} predicates and the initial state predicate of the automaton. Likewise, the second method assembles the new goal specification accordingly with the theory illustrated in Section \ref{sec:encoding-goals}. Finally, the third method simply returns the new problem encoded in standard \PDDL.

\subsection{Automa}\label{sec:impl-automa}
In this section, we illustrate the code that handles extended temporal goals treated as automata. More specifically, we talk about the generation of \DFA corresponding to the \LTLf/\PLTLf goal, the parsing and managing of such generated \DFA showing all implemented data structures.

First of all, as stated before, given an \LTLf/\PLTLf goal formula, we employ the \LTLfToDFA tool to generate the \DFA. Secondly, as soon as the \DFA is generated, we parse it with the \texttt{aparser.py} module and then, we instantiate an \texttt{Automa} object for it. In the following, we will discuss more about the \texttt{Automa} class, since the \texttt{aparser.py} module is pretty much the same discussed in Section \ref{sec:janus-impl-automa}.

\begin{lstlisting}[language=Python, style=Python, escapechar = £,  label={code:fond-automa}, caption={The \texttt{Automa} class.}]
...
class Automa:
    def __init__(self, alphabet, states, initial_state, accepting_states,
     transitions):
        self.alphabet = alphabet
        self.states = states
        self.initial_state = initial_state
        self.accepting_states = accepting_states
        self.transitions = transitions
        self.trans_by_dest = self.group_conditions_by_consequence()£\label{line:trans-by-dest}£
        self.validate()
...
    def validate(self):
        self.validate_initial_state()
        self.validate_accepting_states()
        self.valide_transition_start_states()
        self.validate_input_symbols()
        return True

    def __str__(self):
        automa = 'alphabet: {}\n'.format(str(self.alphabet))
        automa += 'states: {}\n'.format(str(self.states))
        automa += 'init_state: {}\n'.format(str(self.initial_state))
        automa += 'accepting_states: {}\n'.format(str(self.accepting_states))
        automa += 'transitions: {}'.format(str(self.transitions))
        return automa

    def create_operators_trans(self, domain_predicates,£\label{line:op-trans}£ grounded_symbols):
        new_operators = []
        my_predicates = []
        for symbol in grounded_symbols:
            my_predicates.append(symbol.name)
        (parameters, obj_mapping) = £\label{line:trans-param}£ self.compute_parameters(domain_predicates, 
        grounded_symbols)
        vars_mapping = self.compute_varsMapping(grounded_symbols,£\label{line:trans-vars-map}£
         obj_mapping)
        my_variables = self.compute_variables(parameters)
        counter = 0
        for destination, source_action in self.trans_by_dest.items():£\label{line:trans-prec-eff}£
            if source_action:
                fluents_list_precond = self.compute_preconditions(source_action,
                 vars_mapping, my_predicates, my_variables)
                if isinstance(fluents_list_precond, FormulaAnd):
                    new_precondition = fluents_list_precond
                else:
                    new_precondition = FormulaAnd([fluents_list_precond] 
                    + [Literal.negative(Predicate('turnDomain'))])
                new_effects = self.compute_effects(destination, my_variables)
                new_operators.append(Action('trans-'+str(counter),
                 parameters, new_precondition, new_effects))
            else:
                pass
            counter += 1
        return (new_operators, parameters)

    def compute_type(self, all_predicates, name, position):
        for predicate in all_predicates:
            if predicate.name == name:
                if predicate.args:
                    return (predicate.args[position].name +
                     ''.join(random.choices(string.digits, k=2)),
                      predicate.args[position].type)
                else:
                    raise ValueError('[ERROR]: Please check the formula')
            else:
                pass

    def compute_parameters(self,domain_predicates, grounded_symbols):
        objs_set = set()
        obj_mapping = {}
        parameters = []
        for symbol in grounded_symbols:
            if symbol.objects:
                i = 0
                for obj in symbol.objects:
                    if obj not in objs_set:
                        objs_set.add(obj)
                        (name_var, type_) = self.compute_type(domain_predicates, 
                        symbol.name, i)
                        obj_mapping[obj] = [name_var, type_]
                        parameters.append(Term.variable(name_var, type_))
                    else:
                        pass
                    i += 1
        return (parameters, obj_mapping)

    def compute_varsMapping(self, grounded_symbols, obj_mapping):
        temp = []
        vars_mapping = {}
        for symbol in grounded_symbols:
            if symbol.objects:
                for obj in symbol.objects:
                    temp.append((obj_mapping[obj][0], obj_mapping[obj][1]))
            else:
                vars_mapping[symbol] = []
            vars_mapping[symbol] = temp
            temp = []
        return vars_mapping

    def compute_preconditions(self, source_action, vars_mapping,
     predicates_name, variables):
        if len(source_action) == 1:
            if self.get_automaton_formula(vars_mapping, predicates_name,
             source_action[0][1]) == []:
                formula = Literal.positive(Predicate('q'+
                str(source_action[0][0]), variables))
            else:
                automaton_state = [Literal.positive(Predicate('q'+
                str(source_action[0][0]), variables))]
                formula = FormulaAnd(automaton_state+
                self.get_automaton_formula(vars_mapping, predicates_name,
                 source_action[0][1])+[Literal.negative(Predicate('turnDomain'))])
        else:
            formula = FormulaOr(self.get_or_conditions(vars_mapping,
             predicates_name, variables, source_action))
        return formula

    def compute_effects(self, destination, variables):
        negated_states = []
        for state in self.states:
            if state != destination:
                negated_states.append(Literal.negative(Predicate('q'+
                str(state), variables)))
            else:
                pass
        automaton_destination = [Literal.positive(Predicate('q'+
        str(destination), variables))]
        turnDomain = [Literal.positive(Predicate('turnDomain'))]
        formula = FormulaAnd(automaton_destination+negated_states+turnDomain)
        return formula

    def get_or_conditions(self, vars_mapping, predicates_name, variables,
     source_action_list):
        items = []
        for source, action in source_action_list:
            formula = self.get_automaton_formula(vars_mapping,
             predicates_name, action)
            if formula == []:
                items.append(Literal.positive(Predicate('q'+str(source),
                 variables)))
            else:
                automaton_state = [Literal.positive(Predicate('q'+
                str(source), variables))]
                items.append(FormulaAnd(automaton_state+
                self.get_automaton_formula(vars_mapping, predicates_name, 
                action)))
        return items

    def get_automaton_formula(self, vars_mapping, predicates_name, action):
        temp = []
        i = 0
        for char in action:
            if char == '1':
 list(vars_mapping)]:
                temp.append(Literal.positive(Predicate(predicates_name[i],
                 [x[0] for x in vars_mapping[list(vars_mapping)[i]]] )))
 temp.append(Literal.positive(Predicate(predicates_name[i])))
            elif char == '0':
                temp.append(Literal.negative(Predicate(predicates_name[i],
                 [x[0] for x in vars_mapping[list(vars_mapping)[i]]] )))
 temp.append(Literal.negative(Predicate(predicates_name[i])))
            else:
                pass
            i += 1
        return temp

    def compute_variables(self, parameters_list):
        my_variables = []
        for param in parameters_list:
            my_variables.append(param.name)
        return my_variables

    def create_dict_by_destination(self):
        trans_by_dest = {}
        for state in self.states:
            trans_by_dest[state] = []
        return trans_by_dest

    def group_conditions_by_consequence(self):
        group_by_dest = self.create_dict_by_destination()
        for source, trans in self.transitions.items():
            i = 0
            for dest in trans.values():
                group_by_dest[dest].append((source, list(trans.keys())[i]))
                i +=1
        return group_by_dest
\end{lstlisting}
In Listing \ref{code:fond-automa}, we have the main data structure representing the \DFA generated by \LTLfToDFA. As soon as an object is instantiated, transitions are grouped by destination state by a method at line \ref{line:trans-by-dest}. This operation is useful to get a compact representation of each \texttt{trans} operator created. We recall that, the \texttt{trans} operator, created in Section \ref{sec:encoding-goals}, is then split in multiple \texttt{trans} operators because not all planners support conditional effects.

The main method of the \texttt{Automa} class is obviously the \texttt{create\_operators\_trans} which gather all other methods. It takes as input the domain predicates and the grounded symbols of the goal formula. Moreover, the method consists of the operations explained theoretically. In particular, we have:
\begin{itemize}
\item it computes all parameters involved by the grounded symbols of the formula, at line \ref{line:trans-param}, using the \texttt{compute\_parameters} method;
\item it implements the function $f$, defined in \ref{plan:mapfunc}, mapping objects to variables at line \ref{line:trans-vars-map};
\item it computes variables;
\item at line \ref{line:trans-prec-eff}, it builds preconditions and effects for each transition of the \DFA;
\item for each \texttt{trans} operator created, it is added to a the list of trans operators.
\end{itemize}

In the next Section, we will see the main module, which implements all the high level procedure illustrated previously in Section \ref{sec:fond-plan-appr}.
\subsection{Main Module}
Here, we describe the main module of the \FONDFOR package. It is called \texttt{fond4ltlfpltl.py} and it contains the principal logic covering the \FONDFOR theoretical approach illustrated in Section \ref{sec:fond-plan-appr}. In Listing \ref{code:fond-main}, we show the implementation.

\begin{lstlisting}[language=Python, style=Python, escapechar = £,  label={code:fond-main}, caption={The \texttt{fond4ltlfpltl.py} module.}]
from fond4ltlfpltl.PDDLparser.parser import MyParser
from ltlf2dfa.Translator import Translator
from ltlf2dfa.DotHandler import DotHandler
from fond4ltlfpltl.AutomaParser.symbol import Symbol
from fond4ltlfpltl.AutomaParser.aparser import parse_dot
import argparse, os, subprocess, copy, re

args_parser = argparse.ArgumentParser(...)£\label{line:main-argparser}£

params = vars(args_parser.parse_args())
pddl_parser = MyParser()

try:
    with open(params['<planning_domain>'], 'r') as f:
        domain = f.read()
        f.close()
    parsed_domain = pddl_parser(domain)£\label{line:main-parse-dom}£
except:
    raise ValueError('[ERROR]: Could not parse domain')

try:
    with open(params['<planning_problem>'], 'r') as f:
        problem = f.read()
        f.close()
    parsed_problem = pddl_parser(problem)£\label{line:main-parse-prob}£
except:
    raise ValueError('[ERROR]: Could not parse problem')
...
try:
    translator = Translator(params['<goal_formula>'])£\label{line:main-dfa}£
    translator.formula_parser()
    translator.translate()
    translator.createMonafile(False)
    translator.invoke_mona()
    dot_handler = DotHandler()
    dot_handler.modify_dot()
    dot_handler.output_dot()
    dfa_automaton = parse_dot("automa.dot")
    operators_trans, parameters = dfa_automaton.create_operators_trans(...)£\label{line:main-transs}£
    os.remove('automa.mona')
    os.remove('automa.dot')
except:
    os.remove('automa.mona')
    os.remove('automa.dot')
    raise ValueError('[ERROR]: Could not create DFA')

old_domain = copy.deepcopy(parsed_domain)

new_domain = parsed_domain.get_new_domain(...)£\label{line:main-new-dom}£
new_problem = parsed_problem.get_new_problem(...)£\label{line:main-new-prob}£

try:
    with open("./new-dom.pddl", 'w+') as dom:
        dom.write(str(new_domain))
        dom.close()
    with open("./new-prob.pddl", 'w+') as prob:
        prob.write(str(new_problem))
        prob.close()
except:
    raise IOError('[ERROR]: Something wrong occurred')
    
...    
\end{lstlisting}
To begin with, the main module accepts as input a \PDDL domain, a \PDDL problem and a goal formula. All these arguments are handled by the argument parser at line \ref{line:main-argparser}.

After gathered all inputs, we proceed by parsing both the \PDDL domain and the \PDDL problem (lines \ref{line:main-parse-dom} and \ref{line:main-parse-prob}). The parsing phase is carried out by module illustrated in Section \ref{sec:impl-pddl}.

Then, we translate the \LTLf/\PLTLf goal formula into the corresponding \DFA employing \LTLfToDFA. The code that is in charge of doing that starts at line \ref{line:main-dfa}. Once the \DFA is built, we can construct the new \texttt{trans} operator at line \ref{line:main-transs}.

Consequently, we put all things together and we create the new domain $\D'$ and the problem $\P'$ (lines \ref{line:main-new-dom} and \ref{line:main-new-prob}). Finally, we invoke the FOND-SAT planner feeding it with $\D'$ and $\P'$. If a strong plan is found we obtain it in a file on the working directory.

